Grid Optimal Integration of Power Ships

Power-generating ships or Power Ships (PSs) are considered one of the largest mobile energy resources. In this paper, a model is proposed to evaluate the integration of PSs into power grid operations. The model optimally coordinates the ships to enhance the grid objective; its solution provides optimal generation resource scheduling, as well as optimal scheduling and routing of the ships. IEEE 6-bus and IEEE 118-bus case studies were considered to model the system and to validate the effectiveness of the proposed model.

==> refe.tex <==
@article{1,
author = {Y. Sun and Z. Li and W. Tian and M. Shahidehpour},
journal = {IEEE Transactions on Power Systems},
number = {6},
pages = {4348-4356},
title = {A Lagrangian Decomposition Approach to Energy Storage Transportation Scheduling in Power Systems},
volume = {31},
year = {2016},
}

@article{2,
author = {Y. Sun and Z. Li and M. Shahidehpour and B. Ai},
journal = {IEEE Transactions on Smart Grid},
number = {5},
pages = {2395-2402},
title = {Battery-Based Energy Storage Transportation for Enhancing Power System Economics and Security},
volume = {6},
year = {2015},
}





@article{3,
   author = "Joseph {Czyzyk} and Michael P. {Mesnier} and Jorge J. {Mor{\'{e}}}",
   title ="The NEOS Server",
   journal = "IEEE Journal on Computational Science and Engineering",
   year = 1998,
   volume = "5",
   number = "3",
   pages = "68 ?- 75"
}

@techreport{4,
   author = "Elizabeth D. {Dolan}",
   title = "The NEOS Server 4.0 Administrative Guide",
   institution = "Mathematics and Computer Science Division, Argonne National Laboratory",
   year = "2001",
   type = "Technical Memorandum",
   number = "ANL/MCS-TM-250"
}

@incollection{5a,
   author = "William {Gropp} and Jorge J. {Mor{\'{e}}}",
   title = "Optimization Environments and the NEOS Server",
   booktitle="Approximation Theory and Optimization",
   editor = "Martin D. {Buhman} and Arieh {Iserles}",
   publisher = "Cambridge University Press",
   year = "1997",
   pages = "167 -- 182"
}


@article{sp04,
author = {M. Spivey and W. Powell},
journal = {Transportation Science},
number = {4},
pages = {399-419},
title = {The Dynamic Assignment Problem},
volume = {38},
year = {2004},
}




@article{kt13,
author = {S. Krumke and C. Thielen},
journal = {European Journal of Operational Research},
number = {1},
pages = {46-55},
title = {The generalized assignment problem with minimum quantities},
volume = {228},
year = {2013},
}

@unpublished{,
url = {https://www.maritime-executive.com/article/japan-offers-ship-based-lng-power-generation-for-islands},
}

@article{5,
author = {L. Moccia and J. Cordeau and M. Monaco and M. Sammarra},
journal = {Computers & Operations Research},
number = {9},
pages = {2670-2681},
title = {A column generation heuristic for a dynamic generalized assignment problem},
volume = {36},
year = {2009},
}

@article{6,
author = {J. Tang and B. Xiong and Y. Huang and C. Yuan and G. Su},
journal = {The Journal of Engineering},
number = {13},
pages = {1511-1514},
title = {Optimal configuration of energy storage system based on frequency hierarchical control in ship power system with solar photovoltaic plant},
volume = {2017},
year = {2017},
}

@article{7,
author = {A. Frances-Roger and A. Ge Anvari-Moghaddam and E. Rodriguez-Diaz and J. Ge Vasquez and J. Ge Guerrero and J. Uceda},
journal = {IEEE Transactions on Industrial Informatics, pp},
pages = {1-1},
title = {Dynamic Assessment of COTS Converters-based DC Integrated Power Systems in Electric Ships},
year = {2018},
}

@article{8,
author = {M. Babaei and J. Shi and S. Abdelwahed},
journal = {IEEE Access},
pages = {9430-9441},
title = {A Survey on Fault Detection, Isolation, and Reconfiguration Methods in Electric Ship Power Systems},
volume = {6},
year = {2018},
}

@article{9,
author = {C. Lashway and A. Elsayed and O. Mohammed},
journal = {Electric Power Systems Research},
pages = {50-62},
title = {Hybrid energy storage management in ship power systems with multiple pulsed loads},
volume = {141},
year = {2016},
}

@article{10,
author = {K. Huang and S. Srivastava and D. Cartes and L. Sun},
journal = {Electric Power Systems Research},
number = {4},
pages = {550-556},
title = {Market-based multiagent system for reconfiguration of shipboard power systems},
volume = {79},
year = {2009},
}

@article{12,
author = {S. Sarin and H. Sherali and S. Kim},
journal = {Naval Research Logistics (NRL)},
number = {2},
pages = {131-143},
title = {A branch-and-price approach for the stochastic generalized assignment problem},
volume = {61},
year = {2014},
}

@article{13,
author = {T. Chang},
journal = {IEEE Transactions on Signal Processing},
number = {14},
pages = {3719-3734},
title = {A Proximal Dual Consensus ADMM Method for Multi-Agent Constrained Optimization},
volume = {64},
year = {2016},
}

@article{14,
author = {S. Boyd},
journal = {Foundations and Trends� in Machine Learning},
number = {1},
pages = {1-122},
title = {Distributed Optimization and Statistical Learning via the Alternating Direction Method of Multipliers},
volume = {3},
year = {2010},
}

@article{15,
author = {R. Paudel},
journal = {Economic Papers: A journal of applied economics and policy},
number = {4},
pages = {339-361},
title = {Economic Growth in Developing Countries: Is Landlockedness Destiny?},
volume = {33},
year = {2014},
}

@article{16,
author = {P. Kotrajaras and B. Tubtimtong and P. Wiboonchutikula},
journal = {ASEAN ECONOMIC BULLETIN},
pages = {2},
title = {Does FDI Enhance Economic Growth?-New Evidence From East Asia},
volume = {28},
year = {2011},
unidentified = {p. 183},
}

@unpublished{17,
url = {https://www.thoughtco.com/landlocked-countries-1435421},
}

@article{18,
author = {G. Sulligoi and A. Vicenzutti and R. Menis},
journal = {IEEE Transactions on Transportation Electrification},
number = {4},
pages = {507-521},
title = {All-Electric Ship Design: From Electrical Propulsion to Integrated Electrical and Electronic Power Systems},
volume = {2},
year = {2016},
}

@unpublished{19,
url = {http://www.karadenizenergy.com/en/Web/Page/78},
}

@article{kdbd17,
author = {M. Khooban and T. Dragicevic and F. Blaabjerg and M. Delimar},
journal = {IEEE Transactions on Sustainable Energy, pp},
pages = {1-1},
title = {Shipboard Microgrids: A Novel Approach to Load Frequency Control},
year = {2017},
}

@article{lwbzv12,
author = {C. Liu and J. Wang and A. Botterud and Y. Zhou and A. Vyas},
journal = {Smart Grid},
month = {June},
pages = {2},
title = {“Assessment of impacts of PHEV charging patterns on wind-thermal scheduling by stochastic unit commitment,” IEEE Trans},
volume = {3},
year = {2012},
unidentified = {pp. 675–683},
}

@inproceedings{kg13,
address = {Manhattan, KS, USA pp. 1–6},
author = {I. Krad and D. W. Gao},
booktitle = {” in Proc. North Amer. Power Symp},
month = {September},
publisher = {NAPS)},
title = {“Impact of PHEV on reserve scheduling: A MILP-SCUC method},
year = {2013},
}

@article{kws12,
author = {Khodayar, Mohammad E. and Lei Wu and Mohammad Shahidehpour},
journal = {IEEE Transactions on Smart Grid},
number = {3},
pages = {1271-1279},
title = {Hourly coordination of electric vehicle operation and volatile wind power generation in SCUC},
volume = {3},
year = {2012},
}

@article{kwl13,
author = {Khodayar, Mohammad E. and Lei Wu and Zuyi Li.},
journal = {IEEE Transactions on Smart Grid},
number = {2},
pages = {779-788},
title = {Electric vehicle mobility in transmission-constrained hourly power generation scheduling},
volume = {4},
year = {2013},
}

@article{z11,
author = {Zhou, Chengke and others},
journal = {IEEE Transactions on Energy Conversion},
number = {4},
pages = {1041-1050},
title = {Modeling of the cost of EV battery wear due to V2G application in power systems},
volume = {26},
year = {2011},
}

@unpublished{w18,
author = {Wang, Gang and others},
note = {Energies 11.2 : 435},
title = {Network-Constrained Unit Commitment Based on Reserve Models Fully Considering the Stochastic Characteristics of Wind Power},
year = {2018},
}

@article{f16,
author = {Fu, Yong and others},
journal = {IEEE Transactions on Sustainable Energy},
number = {2},
pages = {535-545},
title = {Integration of large-scale offshore wind energy via VSC-HVDC in day-ahead scheduling},
volume = {7},
year = {2016},
}

@article{mzk02,
author = {Momoh, J. A. and J. Z. Zhu and S. S. Kaddah},
journal = {Electric Power Systems Research},
number = {3},
pages = {145-152},
title = {Optimal load shedding study of naval-ship power system using the Everett optimization technique},
volume = {60},
year = {2002},
}

@article{awcgsj17,
author = {Mahnoosh Alizadeh and Hoi-To Wai and Mainak Chowdhury and Andrea Goldsmith and Anna Scaglione and Tara Javidi},
journal = {Control of Network Systems IEEE Transactions on},
pages = {2325-5870},
title = {Optimal Pricing to Manage Electric Vehicles in Coupled Power and Transportation Networks},
volume = {4},
year = {2017},
unidentified = {vol. pp. 863-875 ISSN},
}

@article{cmm98,
author = {Czyzyk, Joseph and Michael P. Mesnier and Jorge J. Moré},
journal = {IEEE Computational Science and Engineering},
number = {3},
pages = {68-75},
title = {The NEOS server},
volume = {5},
year = {1998},
}

@incollection{gm97,
author = {Gropp, William and Jorge Moré},
booktitle = {Approximation theory and optimization},
pages = {167-182},
title = {Optimization environments and the NEOS server},
year = {1997},
}


